Logical Signal Processing: a Fourier Analysis of Temporal Logic

What is the frequency content of temporal logic formulas? That is, when we monitor a signal against a formula, which frequency bands of the signal are relevant to the logic and should be preserved, and which can be safely discarded? This question is relevant whenever signals are filtered or compressed before being monitored, which is almost always the case for analog signals. To answer this question, we focus on monitors that measure the robustness of a signal relative to a specification in Signal Temporal Logic. We prove that robustness monitors can be modeled using Volterra series. We then study the Fourier transforms of these Volterra representations, and provide a method to derive the Fourier transforms of entire formulas. We also make explicit the measurement process in temporal logic and re-define it on the basis of distributions to make it compatible with measurements in signal processing. Experiments illustrate these results. Beyond compression, this work enables the integration of temporal logic monitoring into common signal processing toolchains as just another signal processing operation, and enables a common formalism to study both logical and non-logical operations in the frequency domain, which we refer to as Logical Signal Processing.

==> stash <==
%\subsection{GFRFs of basic operators}
%\label{sec:exp gfrf basic}
%For reference, Fig.~\ref{fig:naked} shows the GFRF spectra (i.e. the magnitudes $|H_n|$) of some of the basic operators in Eq.~\eqref{eq:basic ops}.
%\begin{figure}[t]
%	\centering
%	\includegraphics[width=0.8\linewidth]{figs/naked}
%	\caption{Fourier spectra for some basic operators. For $|H_2|$ the colorbar provides the values (colors in digital copy). (a)  $H_1$ for $\Nlo_f$ with Gaussian atom (only half-period shown). (b)-(d) $|H_1|, |H_2|, |H_3(\cdot,\cdot,1.6)|$ for $\Nonce_{[0.5,0.8]}$, used in modeling Once. (e)-(f) $|H_1|$ and $|H_2|$ for $\Nmax$ used in modeling Or. (g)-(h)  $|H_1|$ and $|H_2|$ for $\Nhist_{[0.5,0.8]}$ used in modeling Historically.}
%	\label{fig:naked}
%\end{figure}


%We approximated $\rob_{\psi_T}$ with a Volterra series, with a maximum relative approximation error of $\approx 10^{-12}$.
%Intuitively, we expect the GFRFs to vary with $T$: at small $T$, high-frequency variations matter: long-range effects take more than $T$ time units to happen and do not affect the formula's robustness or truth value. 
%As $T$ increases the formula also incorporates longer-range variations, as can be seen indeed in Fig.~\ref{fig:once T}(a) middle pane or (b) middle pane.
%Generally however, it is hard to guess, a priori, which frequencies actually matter.
%Intuition quickly breaks down and a \textit{rigorous, quantitative} analysis is needed. 
%Volterra series provide this analysis, as illustrated in Fig.~\ref{fig:once T}.
%We note that at the largest value of $T = 1.0$, both $H_1$ and $H_2$ are identically zero ((a) and (b)), but the higher-order spectra in (c) are non-zero.
%What might explain this? 
%We reason as follows: operator $\rob_{\LTLonce p}$ takes the max of $\rob_p(\sttraj)$ over $[0.5,T]$, and the max operator can `remember' any event in its window $[0.5,T]$.
%So over a larger interval, its output is affected by high-frequency events (happening over a short period of time) \textit{and} low-frequency events (happening over a longer period of time). 
%This manifests itself, quantitatively, in the GFRF spectrum, where higher-order GFRFs $H_n$ weigh the products of $X(\omega)$ over several frequencies, small and large, as per Eq.~\eqref{eq:GFRF def}.
%Depending on the weight $H_n(\omega_1,\ldots,\omega_n)$ given to $\prod_{j=1}^nX(\omega_j)$, that combination of frequencies affects the output more or less.
%This kind of analysis, and its quantitative rigor, are simply not possible without an explicit Fourier domain model of temporal logic.
%
%\begin{figure*}[t!]
%	\centering
%	\begin{subfigure}[t]{0.5\textwidth}
%		\centering
%		\includegraphics[height=1.3in]{figs/once-varyingT-1D}
%		\caption{$|H_1|$ for three values of $T$}
%	\end{subfigure}%
%	~ 
%	\begin{subfigure}[t]{0.5\textwidth}
%		\centering
%		\includegraphics[height=1.3in]{figs/once-varyingT-2D}
%		\caption{$|H_2|$ for three values of $T$ for three values of $T$.}
%	\end{subfigure}
%	\\ \vspace{0.5cm}
%	\begin{subfigure}[t]{0.6\textwidth}
%			\centering
%			\includegraphics[scale=0.4]{figs/once-varyingT-3D}
%			\caption{Slice $|H_3(\cdot,\cdot,0.78)|$ of $|H_3|$.}
%	\end{subfigure}
%	\caption{GFRF spectra for Once$[0, T]$ for three values of $T\in \{0.6,0.8,1\}$. (Colors in digital copy). $H_1 = H_2 \equiv 0$ for the widest interval [0.5,1.0], but $H_3\neq 0$, indicating that third-order (and higher) effects dominate at wider time intervals.}
%	\label{fig:once T}
%\end{figure*}

%\begin{figure}[t]
%	\centering
%	\includegraphics[scale=0.075]{figs/fig9_H1H2H3H4forphi}
%	\caption{$|H1|$,$|H_2|$ and a slice of $|H_3|$ and $|H_4|$ for $\varphi_{T}$}
%	\label{fig:phie gfrf}
%\end{figure}
